SPACE-SET: Staged Pixel-Space Adaptation of Conditioning and EO Generation for Low-Step SAR-to-EO Translation

Latent generative models have shown promise in SAR-to-Electro-Optical Translation (SET), but their reliance on variational autoencoders (VAEs) can limit fine-grained fidelity and low-step inference efficiency. Recent advances in pixel-space diffusion, particularly direct clean-image prediction from noisy pixels, have renewed interest in VAE-free generation and motivated adapting pretrained latent generators. We introduce SPACE-SET (Staged Pixel-Space Adaptation of Conditioning and EO Generation for SAR-to-EO Translation), a staged framework that converts a pretrained latent generator into a VAE-free pixel-space model. To avoid disrupting pretrained representations through simultaneous modality conversion, EO Pixel Transfer (EPT) first adapts the EO generation pathway to pixel space while preserving the pretrained SAR conditioning pathway. SAR Pixel Adaptation (SPA) then converts the SAR conditioning pathway and jointly adapts the generator using pixel-wise uncertainty flow matching (PUFM) and Context-Preserving Distillation (CPD) from the EPT teacher. Both phases share a three-stage curriculum progressing from flow learning and representation alignment to perceptual and adversarial supervision. Low-Step Flow Adaptation (LFA) then separately fine-tunes one- and two-step generators from the SPA model under teacher guidance. Extensive experiments show that our two-step generator leads on four of five quality metrics on QXS-SAROPT, while our one-step generator maintains competitive translation quality with 76.07 times faster inference than a state-of-the-art SET baseline.

==> latexmkrc <==
# Build the main paper's cross-reference data when supplementary.tex is selected.
# Use a separate job name and output directory even when Overleaf calls both
# roots "output". The nested latexmk checks all inputs and reuses its cache.
if (grep { m{(?:^|[/\\])supplementary(?:\.tex)?$}i } @ARGV) {
    my $status = system('latexmk', '-pdf', '-interaction=nonstopmode',
                        '-halt-on-error', '-auxdir=main-ref-build', '-outdir=main-ref-build',
                        '-jobname=main', 'main.tex');
    die "Could not build the reference data from main.tex.\n" if $status != 0;
}

